Data-driven 6D Pose Tracking by Calibrating Image Residuals in Synthetic Domains

Tracking the 6D pose of objects in video sequences is important for robot manipulation. This work presents se(3)-TrackNet, a data-driven optimization approach for long term, 6D pose tracking. It aims to identify the optimal relative pose given the current RGB-D observation and a synthetic image conditioned on the previous best estimate and the object's model. The key contribution in this context is a novel neural network architecture, which appropriately disentangles the feature encoding to help reduce domain shift, and an effective 3D orientation representation via Lie Algebra. Consequently, even when the network is trained solely with synthetic data can work effectively over real images. Comprehensive experiments over multiple benchmarks show se(3)-TrackNet achieves consistently robust estimates and outperforms alternatives, even though they have been trained with real images. The approach runs in real time at 90.9Hz. Code, data and supplementary video for this project are available at https://github.com/wenbowen123/iros20-6d-pose-tracking

==> alg/sampling.tex <==
$T_{t-1}$: previous frame estimated pose \\
$N$: number of particles to sample \\
$I_{t}$: currently observed RGBD image \\
$M$: object CAD model \\
$P_{scene}$: currently observed point cloud (converted from RGBD image) \\

\begin{algorithm}[h]
\label{alg_base_sample}

\caption{{\sc SAMPLE\_INFERENCE\ ($T_{t-1}$,$N$,$I_{t}$,$M$,$P_{scene}$)} }
$LCP_{best} \gets 0$ \;
$T_{t} \gets I_{4\times 4} $\;
\For{$i\gets0$ \KwTo  $N$ }
{
    sample pose $T_{t-1}^{i}$ by adding purturbation to $T_{t-1}$ \;
    render image $I^{i}$ using pose $T_{t-1}^{i}$ \;
    \tcc{neural net predict relative transform}
    $\bigtriangleup T$ \gets $f(I^{i},I_{t})$ \; 
    $T_t^{i} \gets \bigtriangleup T \cdot T_{t-1}$ \;
    $M^i \gets transformation(M,T_t^{i}$) \;
    $LCP^{i} \gets evaluate\_pose\_score(M^i,P_{scene}$) \;

  \If {$LCP^{i} > LCP_{best}$}{
    $LCP_{best} \gets LCP^{i}$ \;
    $T_{t} \gets T_t^{i}$ \;
  }
}

\end{algorithm}


==> sections/conclusion.tex <==
This work presents a framework for efficient and robust long-term 6D object pose tracking. A novel neural network architecture $se(3)$-TrackNet is proposed that allows training on synthetic datasets that transfers robustly to real world data. A combination of design choices for the network and the Lie Algebra representation for learning residual poses during pose tracking result in highly desirable performance validated by extensive experiments. The pose tracking process operates at approximately 90.90 fps, which is significantly higher than alternatives. An additional dataset is proposed to address the lack of an object tracking benchmark in the robotics manipulation context. $se(3)$-TrackNet is shown to be robust under large occlusions and sudden re-orientations introduced in the dataset, which challenge competing approaches. Despite these desirable properties for the proposed network, a limitation is that an object CAD model is required. The future objective is to achieve similar performance for category-level 6D pose tracking.

==> tables/dataset_summary.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
%                                                                           & YCB Video                                                                                             & Choi's                                                                   & T-LESS                                                                   & Issac's                                                                        & Lee's                                                                  & Krull's                                                                & Moving-YCB (ours)                                                                       \\ \hline
% camera used                                                                & RGBD                                                                                                  & RGBD                                                                     & RGBD                                                                     & Depth                                                                          & RGBD                                                                   & RGBD                                                                   & RGBD                                                                                    \\ \hline
% domain                                                                     & real                                                                                                  & synthetic                                                                & real                                                                     & real                                                                           & real                                                                   & real                                                                   & real                                                                                    \\ \hline
% scenario                                                                   & \begin{tabular}[c]{@{}c@{}}moving camera, \\ static objects\end{tabular}                              & \begin{tabular}[c]{@{}c@{}}moving camera, \\ static objects\end{tabular} & \begin{tabular}[c]{@{}c@{}}moving camera, \\ static objects\end{tabular} & \begin{tabular}[c]{@{}c@{}}moving object,\\ static camera\end{tabular}         & \begin{tabular}[c]{@{}c@{}}moving object,\\ static camera\end{tabular} & \begin{tabular}[c]{@{}c@{}}moving object,\\ static camera\end{tabular} & \begin{tabular}[c]{@{}c@{}}moving object,\\ static camera\end{tabular}                  \\ \hline
% object models                                                              & precisely scanned                                                                                     & reconstructed,not precise                                                & precisely scanned                                                        & no texture                                                                     & some have no texture                                                   & reconstructed,not precise                                              & precisely scanned                                                                       \\ \hline
% object categories                                                          & 21                                                                                                    & 4                                                                        & 30                                                                       & 6                                                                              & 8                                                                      & 4                                                                      &                                                                                         \\ \hline
% \begin{tabular}[c]{@{}c@{}}number of videos \\ for evaluation\end{tabular} & 12                                                                                                    & 4                                                                        & 20                                                                       & 37                                                                             & 8                                                                      & 8                                                                      &                                                                                         \\ \hline
% manipulator                                                                & -                                                                                                     & -                                                                        & -                                                                        & human hand                                                                     & human hand                                                             & human hand                                                             & \begin{tabular}[c]{@{}c@{}}vaccum gripper, Yale Hand T42, \\ Robotiq 2F-85\end{tabular} \\ \hline
% pose annotation                                                            & \begin{tabular}[c]{@{}c@{}}inferred from \\ camera trajectory \\ via global optimization\end{tabular} & from simulator                                                           & manually refined                                                         & \begin{tabular}[c]{@{}c@{}}acquired from motion \\ capture system\end{tabular} & manually refined                                                       & manually refined                                                       & manually refined                                                                        \\ \hline
% \end{tabular}%
% }
% % \caption{}
% \label{tab:dataset_compare}
% \end{table*}
